Probing spatial variation of magnetic order in strained SrMnO$_3$ thin films using Spin Hall Magnetoresistance

SrMnO$_{3}$ (SMO) is a magnetic insulator and predicted to exhibit a multiferroic phase upon straining. Strained films of SMO display a wide range of magnetic orders, ranging from G-type to C-and A-type, indicative of competing magnetic interactions. The potential of spin Hall magnetoresistance (SMR) is exploited as an electrical probe for detecting surface magnetic order, to read surface magnetic moments in SMO and its spatial variation, by designing and positioning electrodes of different sizes on the film. The findings demonstrate antiferromagnetic domains with different magnetocrystalline anisotropies along with a ferromagnetic order, where the magnetization arises from double exchange mediated ferromagnetic order and canted antiferromagnetic moments. Further, from a complete analysis of the SMR, a predominance of antiferromagnetic domain sizes of 3.5 $\mu$m$^2$ is extracted. This work enhances the applicability of SMR in unraveling the richness of correlation effects in complex oxides, as manifested by the detection of coexisting and competing ground states and lays the foundation for the study of magnon transport for different magnetoelectric based computing applications.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
